Towards Runtime Adaptation of Actor Systems

In this dissertation we focus on providing effective adaptations that can be localised and applied to specific concurrent actors, thereby only causing a temporary disruption to the parts of the system requiring mitigation, while leaving the rest of the system intact. We make the application of localised adaptations efficient through incremental synchronisation, whereby the specifier can strategically suspend specific parts of the system, whenever this is strictly required for ensuring that adaptations are effectively applied. We also study static analysis techniques to determine whether the specified incremental synchronisation is in some sense adequate for local adaptations to be carried out. We thus identify a number of generic adaptations that can be applied to any actor system, regardless of its design and the code that it executes. We implement the identified adaptations as an extension of an existing Runtime Verification tool for actor-systems, thereby creating a RA framework for monitoring and mitigating actor systems. In parallel to our implementation we also develop a formal model of our RA framework that further serves to guide our implementation. This model also enables us to better understand the subtle errors that erroneously specified adaptation scripts may introduce. We thus develop a static type system for detecting and rejecting erroneous adaptation scripts prior to deployment, thereby providing the specifier with assistance for writing valid scripts. Although the static typesystem analyses scripts with respect to certain assumptions, we do not assume that the monitored system abides by these assumptions. We therefore augment our RA framework with dynamic checks for halting monitoring whenever the system deviates from our assumption. Based on this dynamically checked model of our RA framework, we prove type soundness for our static type system.

==> 4.syn-asyn/sections/hybrid.tex <==

Despite the benefits of synchronous instrumentation, the associated overheads obtained from our preliminary results can make it infeasible in practice.  We therefore devise an alternative instrumentation strategy  with the aim of guaranteeing timely violation detections while incurring lower overheads that are closer to those incurred by asynchronous instrumentation.  
The main idea is to move away from synchronous instrumentation monitoring (SMSI), towards \emph{synchronous detection monitoring} (AMSD) given that, in order to attain timely detections, the instrumentation need not require the system to execute in lockstep with the monitor for \emph{every} monitored event leading to the violation. Instead, (expensive) synchronous event monitoring can be limited to \emph{critical events}, (\ie events \emph{preceeding} a violation), thereby letting the system execute in decoupled fashion otherwise. Intuitively, for the logic of \figref{fig:logic}  these critical events are necessity actions preceeding (directly or indirectly) a \mfls\ forumla.  
%
%From the preliminary results of \secref{sec:synchr-instr} it transpires that synchronous monitoring of events is more expensive than asynchronous event monitoring.  For instance, from \figref{fig:sync_protocol} one can see that  every synchronous monitored event causes the system execution to incur a responsiveness penalty waiting for the monitor to acknowledge back; by contrast,  the system is decoupled from the monitor when events are monitored asynchronously.   

\begin{example}\label{ex:hybrid-instrumentation}
  Recall property (\ref{eq:7:language}) from \exref{ex:simple-formula}.  In order to synchronously detect a violation in this property, only action $\mnec{\msendD{\eatom{server}}{y\!}{\!z}}{}$ needs to be synchronously monitored, since it precedes a \mfls\ forumla (interposed by a conjunction and an if-statement). Action $\mnec{\mrecv{\eatom{server}}{\etuple{\eatom{succ},x,y}}}{}$
  can however be monitored for asynchronously, without affecting the timeliness of detections. \bqed
\end{example}


\subsection{Logic Extensions}
\label{sec:logic-extensions}

We extend the syntax of \detecterGen's logic introduced in \secref{sec:language} by two constructs: a \emph{synchronous false} formula and a \emph{synchronous necessity} formula with a semantics analogous to  that of \mfls\ and \mnec{\actE}{\hV} \resp (see \figref{fig:logic})
\begin{align*}
    \hV,\hVV \in \FRM & \;\bnfdef\; \ldots \;\bnfsep\; \msfls  \quad \emph{(synchronous false)} \;\bnfsep\;  \msnec{\actE}{\hV} \quad \emph{(synchronous necessity)} 
\end{align*}
In the extended logic, formulas carry additional  instrumentation information relating to how they need to be runtime-monitored: by default, all the monitoring is asynchronous, unless one specifies that  a violation is to be synchronously monitored,  \msfls, or that a particular event needs to be synchronously monitored,  \msnec{\actE}{\hV}. Note that synchronous necessities can be used to engineer synchronisation checkpoints (\ie to encode AMC) during periods where the system is not required to be immediately responsive at which point a monitor is allowed to catch up with a system execution, similar to what is presented in \cite{CP12FF}.   

\begin{example} \label{ex:synch-asynch}  We can refine property~\eqref{eq:7:language} as shown below, whereby we distinguish between two kinds of violations, \ie return values $z$ that are less than $x+1$ and return values that are greater than $x+1$, and require the latter violations to be detected in synchronous fashion.\\
  \begin{minipage}[c]{0.90\linewidth}
   \begin{equation*}\setstretch{1}
    \mmax{\hVarX}{\mnec{\mrecv{\eatom{server}}{\etuple{\eatom{succ},x,y}}}{\;\mnec{\msendD{\eatom{server}}{y}{z}}{\;
          \left(
            \begin{array}{l}
              {(\mbool{(z\!=\!x\!+\!1)}{\hVarX\,})} \\
              \quad \mand \;
                  (\mbool{(z< x\!+\!1)}{\mfls\,})
                \\\quad \mand\;
                  (\mbool{(z > x\!+\!1)}{\msfls\,})                
            \end{array}
          \right)
        }}} 
  \end{equation*}
\end{minipage}
\begin{minipage}[l]{0.09\linewidth}
\vspace{1.3cm}
  \bqed
\end{minipage}
\end{example}


The new monitor synthesis algorithm requires a pre-processing phase to determine which events are to be synchronously monitored in order to implement a synchronous fail. For instance, formulas $\mnec{\patE}{\msfls}$ and $\msnec{\patE}{\mfls}$ are both monitored in the same way, in fact the pre-processing phase encodes the former into the latter. In general, however, determining which actions to synchronously monitor for implementing a synchronous fail is not as straightforward, since the $\msfls$ and the first necessity formula preceding this $\msfls$ may be interposed by intermediate formulas such as conjunctions and if-statements (as in the property of \exref{ex:synch-asynch}). In such a case the compiler inspects each if-statement and checks whether there exists at least \emph{one} if-statement that leads directly to a synchronous fail, i.e., {\mbool{b}{\msfls}}, and if so, the action specified in the necessity is synchronously monitored. In hybrid monitoring, both synchronous and asynchronous event monitoring require code instrumentation, as shown in \figref{fig:hybrid_protocol}.  \emph{Asynchronous} events inject advice functions sending a monitor message to the monitor containing the event details and a \emph{null} nonce, \emph{without blocking} the system; upon receiving a null nonce, the monitor determines that it does not need to send an acknowledgment back to the system. \emph{Synchronous} actions are implemented as per synchronous instrumentation (see \secref{fig:sync_protocol}), where \emph{fresh} nonces indicates the monitor that it needs to acknowledge back.

%    In contrast to \cite{Fra:Sey:13},  both synchronous   \emph{and} asynchronous  event monitoring employ instrumentation through code injection at source level through AOP techniques.  % in this hybrid instrumentation.
% The type of instrumentation however differs between the two modes, as shown in  \figref{fig:hybrid_protocol}.   


%\begin{figure}[t]%% VERSION 4
%  \centering
%  \begin{tikzpicture}[>=latex,auto,thick]
%    \begin{scope}[draw=blue!50,fill=blue!20,minimum size=0.8cm]
%      \node (sys) at ( -1,1) [shape=rectangle,draw,fill,text width=4cm, minimum height = 3cm, text centered] 
%          {...\\ Event e1 occurs;\\ Get data d1 from e1;\\...\\Event e2 occurs;\\ Get data d2 from e2;\\...\\Event e3 occurs;\\ Get data d3 from e3;\\Block on nonce(e3);\\...\\\; };
%       \node (mon) at ( 8,1) [shape=rectangle,draw,fill,text width=6.65cm, minimum height = 3cm] {$\; $loop(Nonce)\;$\rightarrow$\\$\quad$ if(Nonce $\not{=} null$)\;$\rightarrow$\\ $\qquad$send\_ack(Nonce) \\ $\quad$end, \\ $\quad$\{EVT,Nonce2\} = recv\_event(), \\ $\quad$HasPatternMatched = handle(EVT), \\ $\quad$if(HasPatternMatched) $\rightarrow$ \\ $\qquad$loop(Nonce2); \\ $\quad$else if(Nonce $\not{=} null$)\;$\rightarrow$\\ $\qquad$ send\_ack(Nonce2)\\ $\quad$end. };  
%        \node (sysN) at (-1,4.2) {\textbf{System}}; 
%        \node (monN) at (8,4.2) {\textbf{Monitor}}; 
%    \end{scope}
%       \node (sys1) at (1,2.0){};
%       \node (mon1) at (4.7,2.0){};
%       \node (sys2) at (1,1.0){};
%       \node (mon2) at (4.7,1.0){};
%       \node (sys3) at (1,0){};
%       \node (mon3) at (4.7,0){};
%       \node (sys4) at (1,-0.5){};
%       \node (mon4) at (4.7,-0.5){};
%    \begin{scope}[draw=red,fill=red, dashed]
%      \draw[->] (sys1) to node{\textbf{evt}(d1,null)} (mon1); 
%      \draw[->] (sys2) to node{\textbf{evt}(d2,null)} (mon2); 
%      \draw[->] (sys3) to node{\textbf{evt}(d3,nonce1)} (mon3); 
%      \draw[->] (mon4) to node{\textbf{ack}(nonce1)} (sys4); 
%    \end{scope}
%  \end{tikzpicture}
%  \caption{A high-level depiction of the hybrid monitoring protocol. % Null nonces are not acknowledged by the monitor.
%  }
%       \label{fig:hybrid_protocol}
%\end{figure}

\begin{figure}[t]%% VERSION 4
  \centering
  \begin{tikzpicture}[>=latex,auto,thick]
    \begin{scope}[draw=blue!50,fill=blue!20,minimum size=0.8cm]
      \node (sys) at ( -1,1) [shape=rectangle,draw,fill,text width=4.8cm, minimum height = 3cm, text centered] 
          {...\\ Actor $i$ commits event e1;\\ $i$ gets data d1 from e1;\\...\\Actor $j$ commits event e2;\\ $j$ gets data d2 from e2;\\...\\ Actor $i$ commits event e3;\\ $i$ gets data d3 from e3;\\$i$ blocks on nonce(e3);\\ $i$ unblocks with nonce1;\\...\\\; };
       \node (mon) at ( 8,1) [shape=rectangle,draw,fill,text width=5.6cm, minimum height = 3cm] {\\[1mm]$\; $loop(Nonce)\;$\rightarrow$\\$\quad$ if(Nonce $\not{=} null$)\;$\rightarrow$\\ $\qquad$send\_ack(Nonce) \\ $\quad$end, \\ $\quad$\{Evt,Nonce2\} = recv\_event(), \\ $\quad$PtrnMatch = handle(Evt), \\ $\quad$if(PtrnMatch) $\rightarrow$ \\ $\qquad$loop(Nonce2); \\ $\quad$else if(Nonce $\not{=} null$)\;$\rightarrow$\\ $\qquad$ send\_ack(Nonce2)\\ $\quad$end.\\[2mm]\; };  
        \node (sysN) at (-1,4.5) {\textbf{System}}; 
        \node (monN) at (8,4.5) {\textbf{Monitor}}; 
    \end{scope}
       \node (sys1) at (1.4,3.2){};
       \node (mon1) at (5.2,3.2){};
       \node (sys2) at (1.4,1.5){};
       \node (mon2) at (5.2,1.5){};
       \node (sys3) at (1.4,0){};
       \node (mon3) at (5.2,0){};
       \node (sys4) at (1.4,-0.5){};
       \node (mon4) at (5.2,-0.5){};
    \begin{scope}[draw=red,fill=red, dashed]
      \draw[->] (sys1) to node{\textbf{evt}(d1,null)} (mon1); 
      \draw[->] (sys2) to node{\textbf{evt}(d2,null)} (mon2); 
      \draw[->] (sys3) to node{\textbf{evt}(d3,\{i,nonce1\})} (mon3); 
      \draw[->] (mon4) to node{\textbf{ack}(nonce1)} (sys4); 
    \end{scope}
  \end{tikzpicture}
  \caption{A high-level depiction of the hybrid monitoring protocol. % Null nonces are not acknowledged by the monitor.
  }
       \label{fig:hybrid_protocol}
\end{figure}

\subsection{Evaluation}
\label{sec:evaluation}

Using the extended syntax, we reformulate the security properties used for the evaluation of \secref{sec:preliminary-results} and require violation detections to be synchronous \ie using \msfls\ instead of \mfls.  For instance, from property \eqref{eq:5} we obtain the property below.

\begin{equation} \setstretch{1.1}
\begin{array}{l}
    \mmax{\hVarX}{\big( \\\qquad\msnec{\msendD{\_}{\eatom{AcceptorPid}}{\etuple{handlerPid,\eatom{next},\_}}}\\
      \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws}, \eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},\etuple{\eatom{http\_req},\eatom{GET},\_ ,\_}}}}}\\
    \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws}, \eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h1}}}}\\
    \qquad \vdots \\% \mnec{\mret{handlerPid}{\etuple{\eatom{yaws}, \eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h2}}}}\\
    % \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h3}}}}\\
    % \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h4}}}}\\
    % \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h5}}}}\\
    \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h6}}}}\\
    \qquad
       \mboolE{(\textsl{isMalicious}(h1,h2,h3,h4,h5,h6))}{\;\msfls\;\\\qquad}{\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},\eatom{http\_eoh}}}}}{\;\hVarY}}     \\ \big) }       
\end{array}\label{eq:6}
\end{equation}

\noindent We measure the respective overheads resulting from the hybrid instrumentations over Yaws for varying client loads in terms of 
\begin{itemize} \itemsep0em \setstretch{1}
	\item the average number of \emph{CPU cycles} required per Yaws client request;
	\item the average \emph{memory utilisation} for the Yaws server to respond to batches of client requests; and
	\item the average response time of the (monitored) Yaws server, \ie the time taken for the server to respond to a client request\footnote{In the extended syntax, properties that are exclusively defined in terms of synchronous necessity formulas, \msnec{\actE}{\hV}, yield synchronous monitor instrumentations that are identical to those discussed in \secref{sec:synchr-instr}.}.
\end{itemize}
The experiments were carried out on an Intel Core 2 Duo T6600 processor with 4GB of RAM, running Microsoft Windows 7 and EVM version R16B03. To further confirm the discrepancies between synchronous, hybrid and asynchronous monitoring we run our test-suite and take separate batches of results using $(i)$ unoptimised monitors, $(ii)$ statically optimised monitors and $(iii)$ dynamically optimised monitors. For each property (in our test-suite) and each client load, we take five sets of readings and then average them out. Since results pertaining to a specific monitor optimisation do not show substantial variations when using different properties, we again average the results across all properties and compile them as graphs for each optimisation, so to obtain the graphs shown in \Cref{fig:unopt_results,fig:sopt_results,fig:s+dopt_results}. 

From the graphs in \Cref{fig:unopt_results,fig:sopt_results,fig:s+dopt_results} we see that regardless of how the monitors are optimised \cite{CasFraSaid15}, memory and CPU utilisation suffer from a marginal difference in which the hybrid monitoring overheads generally lie midway between synchronous monitoring, which scored the worst and asynchronous monitoring, which gave the best performance results. A clearer, and more substantial difference is seen in the average time that the server takes to respond to each client request when it is under a certain load. Providing low average response times is imperative in reactive systems (such as webservers) to make sure that the client is served as soon as possible.% to avoid from hindering the operations of the requesting client. 
\figref{fig:unopt_results} shows that unoptimised monitors suffer from a substantial response difference of about 46ms when a synchronously monitored instance of Yaws is placed under the load of 2000 client requests, as compared to its asynchronous counterpart. By contrast hybrid monitoring provided timely detections by suffering only from a 9ms response overhead increase (for the same load) when compared to asynchronous monitoring.  

Furthermore, \cref{fig:sopt_results,fig:s+dopt_results} demonstrate that even though optimisations help in reducing the overall overheads, under a load of 2000 clients synchronous monitoring still fared the worst. In fact this suffers from a 19ms difference (compared to asynchronous) when using statically optimised monitors, and a 9ms difference with dynamically optimised monitors. Contrasting this, the hybrid approach only suffers from a 4ms and 1.5ms response time difference for statically optimised and dynamically optimised monitors respectively.   

\begin{figure}
\centering
	%\input{graphs/UNOPT_CPU_UTIL.tex}
	\input{4.syn-asyn/graphs/UNOPT_CPU_UTIL_PER_REQ.tex}
	\input{4.syn-asyn/graphs/UNOPT_MEM_UTIL.tex}
	\indent\input{4.syn-asyn/graphs/UNOPT_AVG_RESP_TIME.tex}\vspace{-5mm}
	\caption{Performance impact analysis (using unoptimised monitors)}
	\label{fig:unopt_results}
\end{figure}


\begin{figure}
\centering
	%\input{graphs/SOPT_CPU_UTIL.tex}
	\input{4.syn-asyn/graphs/SOPT_CPU_UTIL_PER_REQ.tex}
	\input{4.syn-asyn/graphs/SOPT_MEM_UTIL.tex}
	\indent\input{4.syn-asyn/graphs/SOPT_AVG_RESP_TIME.tex}\vspace{-5mm}
	\caption{Performance impact analysis (using statically optimised monitors)}
	\label{fig:sopt_results}
\end{figure}

\begin{figure}
\centering
	%\input{graphs/S+D_OPT_CPU_UTIL.tex}
	\input{4.syn-asyn/graphs/S+D_OPT_CPU_UTIL_PER_REQ.tex}
	\input{4.syn-asyn/graphs/S+D_OPT_MEM_UTIL.tex}
	\indent\input{4.syn-asyn/graphs/S+D_OPT_AVG_RESP_TIME.tex}\vspace{-5mm}
	\caption{Performance impact analysis (using fully optimised monitors)}
	\label{fig:s+dopt_results}
\end{figure}

==> 4.syn-asyn/sections/yaws-casestudy.tex <==
%%% COMMENT/MOTIVATION ABOUT WHY WE NEED TO USE FUNCTION RETURNS INSTEAD OF RECEIVES 
% The main reason why we used function returns is that in order to receive TCP messages from a connected client, Yaws uses ``inet'' Erlang library which is part of the EVM's kernel. Hence to synchronously monitor these receives directly entails that this kernel library should also be instrumented by the detectEr compiler. This is not suggested as other Erlang applications, that also use the same library, would most probably be negatively affected if the instrumented code is taken out of its monitoring context. Hence by using function returns we could achieve the same result by instrumenting the code of the Yaws server alone.  
%%%

Regardless of the simplicity and elegance of \detecterGen's logic, it turns out that it provides enough expressivity to express a number of safety properties for Yaws, including the Directory Traversal Vulnerability found in earlier versions of the software and reported on the reputable exploit-db website \cite{yaws-exploit-misc} (see App.~\ref{sec:alt-yaws-prop} for details). We here discuss a second safety property for the webserver.

If we assume the existence of a (decidable) predicate called $\textsl{isMalicious}()$, which can determine whether the client will engage in security-breaching activity from the 6 HTTP headers sent to the handler, we can use the logic of \figref{fig:logic} (see \secref{sec:language}) to specify the safety property stated in (\ref{eq:5}).  The property requires that, for \emph{every} client connection established (determined from message $(2)$ of \figref{fig:yaws-protocol} and denoted in property (\ref{eq:5}) as the action $\mnec{\msendD{\_}{\eatom{AcceptorPid}}{\etuple{handID,\eatom{next},\_}}}$) the following subproperty must hold: for \emph{every} HTTP request, the respective headers communicated ($h1$ to $h6$) do not amount to a potentially security-breaching request (as determined by the predicate $\textsl{isMalicious}()$).
\begin{equation} \setstretch{1.1}
\begin{array}{l}
    \mmax{\hVarX}{\big( \\\qquad\mnec{\msendD{\_}{\eatom{AcceptorPid}}{\etuple{handlerPid,\eatom{next},\_}}}\\
      \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws}, \eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},\etuple{\eatom{http\_req},\eatom{GET},\_ ,\_}}}}}\\
    \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws}, \eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h1}}}}\\
    \qquad \mnec{\mret{handlerPid}{\etuple{\eatom{yaws}, \eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h2}}}}\\
     \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h3}}}}\\
     \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h4}}}}\\
     \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h5}}}}\\
    \qquad\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},h6}}}}\\
    \qquad
       \mboolE{(\textsl{isMalicious}(h1,h2,h3,h4,h5,h6))}{\;\mfls\;\\\qquad}{\mnec{\mret{handlerPid}{\etuple{\eatom{yaws},\eatom{do\_recv},\eatom{3},\etuple{\eatom{ok},\eatom{http\_eoh}}}}}{\;\hVarY}}     \\ \big) }       
\end{array}\label{eq:5}
\end{equation}
The logical formula stated in \eqref{eq:5} specifies this property as a recursive formula, $\mmax{\hVarX\!}{(\ldots)}$, whereby the process id of the handler assigned by the acceptor process is pattern-matched with the term variable \emph{handlerPid}. This value is then used to pattern match with the header term variables, \emph{h1} to \emph{h6}, for every iteration of the HTTP request protocol; an if-statement is then used to determine whether these HTTP requests violate the property or not.  We note  that,  whereas the handler messages to the acceptor  are observed \emph{directly} (\ie the output action in the outer recursive formula), the client HTTP messages received by the handler have to be observed \emph{indirectly} through the return values (of the form $\etuple{\eatom{ok},\_}$) of the invoked function \eatom{do\_recv}.\footnote{Defined in module \eatom{yaws} with arity \eatom{3}.}   Instrumentation allowing a direct observation of these  actions is complicated by the fact that the client TCP messages are sent through functions from the \eatom{inet} Erlang library, which is part of the Erlang Virtual Machine kernel.

\subsection{Component-based Monitor Generation}
\label{sec:monit-synth-scal}

Recall that the monitors generated by \detecterGen are \emph{not} monolithic, but instead consist of systems of concurrent (sub)monitors, each analysing different parts of a system under examination.  For instance, in the case of property \eqref{eq:5}, \detecterGen first generates a submonitor that listens for the action $\mnec{\msendD{\,\_\,}{\eatom{AcceptorPid}}{\etuple{handID,\eatom{next},\_}}}$  from the unassigned (free) handler waiting on the TCP port.  Once this action is detected, it spawns a new submonitor to listen for the new handler, while it continues monitoring for the handler that is now assigned to a client.  Thus, after two client connections are accepted, we end up with the configuration depicted in \figref{fig:yaws-monit}.  Note that the submonitors need not communicate with each other since a violation detected by one submonitor immediately means that the global property is violated.  

\begin{figure}[t]
  \centering
  \begin{tikzpicture}[>=latex,auto,thick]
    \begin{scope}[draw=blue!50,fill=blue!20,minimum size=0.8cm]
      \node (client2) at ( 0,4.5) [shape=rectangle,draw,fill] {Client};
      \node (cHandler2) at ( 4,4.5) [shape=rectangle,draw,fill] {Handler};
      \node (mon2) at (8,4.5)  [shape=rectangle,draw] {Monitor};
      
      \node (client) at ( 0,3) [shape=rectangle,draw,fill] {Client};
      \node (cHandler) at ( 4,3) [shape=rectangle,draw,fill] {Handler};
      \node (mon) at (8,3)  [shape=rectangle,draw] {Monitor};
      
      \node (acceptor) at ( 11,3) [shape=rectangle,draw,fill] {Acceptor};  
     \node (newHandler) at ( 4,1.5) [shape=rectangle,draw,fill] {(free) Handler};
     \node (newmon) at (8,1.5)  [shape=rectangle,draw] {Monitor};     
    \end{scope}
   \begin{scope}[draw=black,dashed,minimum size=0.8cm] 
   \end{scope}
    \begin{scope}[draw=red,fill=red]
      \draw[<->] (client) to node{assigned} (cHandler);
      \draw[<->] (client2) to node{assigned} (cHandler2); 
     \end{scope}
    \begin{scope}[draw=black, dashed]
      \draw[<-] (mon) to node{trace} (cHandler);
      \draw[<-] (mon2) to node{trace} (cHandler2);
      \draw[<-] (newmon) to node{trace} (newHandler);
    \end{scope}
  \end{tikzpicture}
  \caption{Component-based Monitoring}
\label{fig:yaws-monit}
\end{figure}
